Incremental Sliding Window Connectivity over Streaming Graphs

We study index-based processing for connectivity queries within sliding windows on streaming graphs. These queries, which determine whether two vertices belong to the same connected component, are fundamental operations in real-time graph data processing and demand high throughput and low latency. While indexing methods that leverage data structures for fully dynamic connectivity can facilitate efficient query processing, they encounter significant challenges with deleting expired edges from the window during window updates. We introduce a novel indexing approach that eliminates the need for physically performing edge deletions. This is achieved through a unique bidirectional incremental computation framework, referred to as the BIC model. The BIC model implements two distinct incremental computations to compute connected components within the window, operating along and against the timeline, respectively. These computations are then merged to efficiently compute queries in the window. We propose techniques for optimized index storage, incremental index updates, and efficient query processing to improve BIC effectiveness. Empirically, BIC achieves a 14$\times$ increase in throughput and a reduction in P95 latency by up to 3900$\times$ when compared to state-of-the-art indexes.

==> sections/colver_letter.tex <==
{\parindent 0cm
\begin{center}
\textbf{\Large Cover Letter \\ Response to Reviewers' Comment}    
\end{center}

We greatly thank the reviewers for the thorough reviews and useful comments. 
% 
We have addressed all reviewers' comments in the revised version. 
We first summarize the changes below. Then, we answer the reviewers' concerns by mentioning the comments and adding our answers. \\
\textbf{Main Changes}:
\begin{itemize}
    \item \textit{Change 1}: In the revised experimental evaluation, we add two new datasets Youtube-Growth (YG) and Semantic-Scholar (SC), which overlap with the most recent baseline D-Tree (\textbf{R3.D5.1}). The new results are presented in Figures \ref{fig:per_throughput}, \ref{fig:per_latency}, \ref{fig:scale_window_size}, \ref{fig:scale_slide_size}, and \ref{fig:scale_workload_size}. Generally, our experimental results do not change over these two new datasets, \textit{i.e.}, BIC significantly outperforms D-Tree in various settings.
    \item \textit{Change 2}: We conduct experiments on memory consumption using all datasets (\textbf{R1.W2\&R3.D4}), including the two new datasets YG and SC. The memory usage results are presented in Figure \ref{fig:per-memory}, where the same settings of window sizes and slide intervals are used. Generally, BIC uses less memory than D-Tree, and BIC uses the least amount of memory among index-based approaches in various settings. 
    \item \textit{Change 3}: We add more clarification and detail to explain our approach and more discussion in experimental results, including why deletion operation is expensive in approaches based on fully dynamic connectivity like D-Tree (\textbf{R1.W1}), how BIC transforms deletion operations into insertion operations (\textbf{R3.D2}), promising research directions of BIC (\textbf{R1.W3\&R1.W4}), more explanation of the running example (\textbf{R3.D1}), pseudocodes of all algorithms in BIC (\textbf{R3.D3}), and experimental result analysis using average distance and diameter of graphs (\textbf{R3.D5.2}).
\end{itemize}

\hfill

\textit{\textbf{\large Meta-Review (MR) Comments:}}

\smallskip
\textit{There are mostly positive, reviews (WA,A,WA) for this submission.
The submission appears to address an interesting problem, is well-written, and presents promising performance (throughput, latency, storage) results on multiple datasets.
Concerns appear to be on some relatively minor presentation issues and a few additional experiments that can further clarify the various aspects of the proposed methodology.
Given these, I am inclined to recommend that this submission goes through a revision cycle.}
\smallskip

\textbf{Answer\&Revision: }
Thank you for offering a revision opportunity to allow us to improve the manuscript. 
We appreciate the thorough and comprehensive reviews and have revised the manuscript accordingly.
Please refer to the summary of \textbf{Main Changes} at the beginning of the letter for an overview.
\smallskip
\smallskip
\smallskip

\textit{\textbf{\large Reviewer \#1 Comments:}}
\smallskip
\smallskip
\smallskip

\textit{\textbf{W1}. The main purpose of the paper is to eliminate the operation of deleting expired edges in maintaining indexes for processing connectivity queries in sliding windows, and repeatedly emphasize that the deletion operation is expensive, but there is a lack of specific examples or more detailed introduction to prove this.
}\\
\textbf{Answer:} 
%Thank you for the comment. 
In general, edge deletion in the data structures for fully dynamic connectivity (FDC) is known to be the most expensive operation for all existing FDC data structures (including the most recent one D-Tree), taking $O(|V|+|E|)$ time in the worst case. This is because these data structures use  spanning trees to represent connected components in the graph. Then, deleting an edge of a spanning tree will first lead to splitting the tree into two sub-trees and then traversing the entire graph to check whether there exists an edge that can reconnect the two sub-trees. This problem is known as searching for a replacement edge, and the worst-case time complexity of the state-of-the-art approach for this problem is $O(|V|+|E|)$.
We discussed fully dynamic connectivity in Section \ref{sec:related_works}. \\
% 
\textbf{Revision:} We add more clarification and also use the running example to explain the problem in Section \ref{sec:intro} (page 2, the left column). We also revise and highlight our discussion in Section \ref{sec:related_works}.
\smallskip
\smallskip
\smallskip

\textit{\textbf{W2}. This paper proposes a method for efficiently storing backward buffer, but it still needs to store a large amount of data. There should be comparative experiments on the memory overhead with other methods.}\\
\textbf{Answer:} 
%Thank you for the comment. 
We have added experiments regarding memory overhead of all approaches in Section \ref{sec:memory_udage}. As shown in these experiments, our approach does not require more storage space, compared to the current state-of-the-art approach, \textit{i.e.}, D-Tree.
This is because D-Tree (or approaches based on FDC data structures) requires storing all the vertices and edges for the graph in each window instance since it stores the spanning forest and also all the non-tree edges, \textit{i.e.}, $O(n + m)$ space.
% 
However, BIC utilizes Union-Find Trees for indexing and storing edges per chunk rather than per window instance.
% 
While the space complexity of BIC is $O(|c|n + m)$,  the memory used to store edges in each chunk is freed after computing the chunk's backward buffer. This process typically reduces the memory requirement to $O(|c|n)$ for most window instances. \\
\textbf{Revision:} We add new experiments on memory consumption and discussion of the results of all approaches using all datasets in Section \ref{sec:memory_udage}. The memory experiments include all settings of our experiments, \textit{i.e.}, a sliding window with a window size of $3$M edges and $150$K edges, sliding windows with a slide size of $1$M edges and different window sizes, and sliding windows with a window size of $80$M edges and different slide sizes, excluding the workload size setting. Workload sizes were omitted as they do not impact memory usage, given that queries are processed through straightforward index lookups. In addition, we add discussion on the space complexity of our approach and compare it to the space complexity of FDC approaches at the end of Section \ref{sec:backward_parallel}. 
\smallskip
\smallskip
\smallskip


\textit{\textbf{W3}. What is the parallel performance of BIC when running on multiple cores? Other approaches should be able to easily support and benefit from parallelism, for example RWC is parallel friendly.}\\
\textbf{Answer:}
Thank you for your insightful comment and the suggestion of a future research direction.
While parallelization presents an interesting avenue, it's important to note that our current model prioritizes continuous processing over graph streams (Section \ref{sec:related_works}), where edges are processed sequentially to enable real-time analysis. In this context, parallelization needs further thought.
% 
In a micro-batching scenario, where streaming data is processed in batches rather than individually, the potential for parallel processing of multiple streaming edges is straightforward.
However, for comparison, it is unclear how to parallelize D-Tree. 
It's worth mentioning that both RWC and our method leverage Union-Find Trees, hinting that existing parallelization techniques for these trees could facilitate the parallelization of BIC. Investigating this promising pathway will be a key focus of our future research.\\
\textbf{Revision:} We add parallelization as one of the future research directions in Section \ref{sec:conclusion}.
\smallskip
\smallskip
\smallskip

\textit{\textbf{W4}. Chunk settings have an important impact on storage and performance. The paper seems to lack introduction and analysis of how to set them.}\\
\textbf{Answer:}
%Thank you for your comment and for highlighting a promising direction for future research. 
The observation of the link between chunk size and performance is indeed correct. In our current study, we concentrate on scenarios where the chunk size matches the window size divided by the slide interval, enabling us to merge a single element from a backward buffer with one from a forward buffer. This approach has already yielded considerable performance enhancements compared to existing methods.
% 
Adjusting the chunk size would necessitate a tailored design for the merging operation within the BIC model, potentially offering further optimization possibilities for both backward and forward buffer computations, thereby enhancing computation efficiency. We are keen to investigate this opportunity in our future work.\\
\textbf{Revision:} We add discussion in Section \ref{sec:bic} (page 4, the right column) to explain the setting of chunk size in this paper and also the study of chunk size as future work in Section \ref{sec:conclusion}.
\smallskip
\smallskip
\smallskip


\textit{\textbf{D1}. Should f1[2] of Q(W3) in Example 4.5 be changed to f2[1]?}\\
\textbf{Answer:} Thank you for carefully reading our manuscript. Yes, it should be $f_2[1]$. \\
\textbf{Revision:} We correct the mistake in Example \ref{example:bic-model}.
\smallskip
\smallskip
\smallskip

\hfill

\textit{\textbf{\large Reviewer \#2 Comments:}}
\smallskip
\smallskip
\smallskip

\textit{\textbf{D1-4}.\\
\textbf{(1)} The paper proposes a number of techniques and insights that are technically interesting.\\
\textbf{(2)} As the source code of the paper is publicly available, everyone can test the results and even experiment with the code.\\
\textbf{(3)} The presentation and the writing of this paper are impressive. It's a model of how a paper should be written: elegant, with nice drawings, many examples, and an intuitive explanation. I appreciate the authors' effort.\\
\textbf{(4)} The experimental results are good and show that the presented techniques work efficiently.}\\
\textbf{Answer:} Thank you very much for your support. We appreciate your understanding of the novelty, the contribution of our approach, and our efforts to improve the readability of the manuscript.

\hfill

\textit{\textbf{\large Reviewer \#3 Comments:}}
\smallskip
\smallskip
\smallskip

\textit{\textbf{W1}. Certain expressions in the manuscript lack clarity and would benefit from additional elaboration to improve readability.}\\
\textbf{Answer\&Revision:} %Thank you for the comment. 
We have revised the manuscript as indicated in the answers to \textbf{D1}, \textbf{D2}, \textbf{D3}, and \textbf{D5.2} below.
\smallskip
\smallskip
\smallskip

\textit{\textbf{W2}. Additional experiments are needed to fully substantiate all the viewpoints presented in the paper.}\\
\textbf{Answer\&Revision:} %Thank you for the comment. 
We have revised the manuscript as indicated  in the answers to \textbf{D4} and \textbf{D5.1} below.
\smallskip
\smallskip
\smallskip

\textit{\textbf{D1}. The depiction of Figure 2 in Section 1 lacks clarity. The meanings of b1[0], b1[1], ... b1[4], and f2[0], f2[1], ... , f2[4] are not elucidated. Furthermore, the importance of Q(W3) = b1[2] $\oplus$ f2[1] is not expounded upon. It is advisable to furnish a brief explanation in the original context or specify where readers can access the clarification to augment the paper's readability.}\\
\textbf{Answer:} %Thank you for the comment. 
Intuitively, $f_2[1]$ captures the connectivity information of edges spanning from $\tau_6$ to $\tau_7$, whereas $b_1[2]$ encompasses the connectivity information of edges from $\tau_3$ to $\tau_5$ (see Section \ref{sec:incremental_connectivity} for details). Consequently, any connectivity query $Q$ over $\window_3$ can be computed by merging these segments of connectivity information (see Section \ref{sec:merging_sub_connectivity} for details). \\
\textbf{Revision:} We add the above discussion in Section \ref{sec:intro} (page 2, the left column).
\smallskip
\smallskip
\smallskip

\textit{\textbf{D2}. The manuscript frequently asserts that the BIC model eliminates the need for deleting expired edges. However, it lacks explicit and straightforward explanation of the transformation from expired edge deletion to insertion. It is recommended to improve clarity and comprehensibility by incorporating illustrative examples into the text.}\\
\textbf{Answer:} %Thank you for the comment. 
Generally, we compute the backward buffer to store the connectivity information for a fragment of the entire window, which allows us to eliminate the need for performing deletion operations.  We use the running example 
in Figures \ref{fig:sliding-window-connectivity} and \ref{fig:bic} to give straightforward explanation. For example, $Q$ over $\window_3$ is computed by merging the segments of connectivity information stored in $f_2[1]$ and $b_1[2]$, respectively. Our approach contrasts with a FDC approach, which necessitates deleting expired edges with $\tau_2$ from and inserting new edges with $\tau_2$ into the index of $W_2$. \\
\textbf{Revision}: We add the above discussion in Section \ref{sec:intro} (page 2, the left column).
\smallskip
\smallskip
\smallskip


\textit{\textbf{D3}. The algorithms outlined in Section 4 and Section 5 would benefit from the inclusion of pseudocode to improve readability, particularly in explaining the calculation of buffer elements and the sub-connectivity merging process.}\\
\textbf{Answer:} %Thank you for the comment. 
We agree that including all of these algorithms would be desirable, but we are facing a serious space problem and there are no suggestions for what can be deleted and we cannot easily identify any discussion we can leave out. The manuscript contains many intuitive and detailed examples, which we believe makes the approach more understandable. Nevertheless, we have taken some measures to include more algorithms.

\textbf{Revision:} 
We provide the pseudocodes of the following algorithms in the appendix of the manuscript: the snapshot isolation approach for storing backward buffers (Algorithm \ref{algo:snapshot_isolation}), the approach for computing AUFTs in backward buffer (Algorithm \ref{algo:augmented_backward_buffer}), the approach for computing edges and intervals using AUFTs (Algorithm \ref{algo:compute_edges_intervals}), the approach for computing BFBGs based on Algorithm \ref{algo:compute_edges_intervals} (Algorithm \ref{algo:compute_bfbg}), and the approach for query processing with the merging process (Algorithm \ref{algo:query_processing}). 
\smallskip
% \smallskip

The full version of our paper is currently available on our GitHub repository \cite{bic-tech}, and we will make it available on arXiv after the final decision. 
\smallskip
\smallskip
\smallskip

\textit{\textbf{D4}. In Section 7, the experiments have illustrated the performance of the proposed method concerning throughput and latency in comparison to state-of-the-art approaches, however, there is a lack of experimental evidence concerning space utilization. It is suggested to incorporate experiments focusing on memory consumption, conducting a comparative analysis of the proposed method's dynamic memory usage against that of state-of-the-art approaches, to provide a comprehensive demonstration of the proposed method's performance.}\\
\textbf{Answer:} 
%Thank you for the comment. 
We have added experiments regarding memory overhead of all approaches in Section \ref{sec:memory_udage}. As shown in these experiments, our approach does not require more storage space, compared to the current state-of-the-art approach, \textit{i.e.}, D-Tree.
This is because D-Tree (or approaches based on FDC data structures) requires storing all the vertices and edges for the graph in each window instance since it stores the spanning forest and also all the non-tree edges, \textit{i.e.}, $O(n + m)$ space.
% 
However, BIC utilizes Union-Find Trees for indexing and storing edges per chunk rather than per window instance.
% 
While the space complexity of BIC is $O(|c|n + m)$,  the memory used to store edges in each chunk is freed after computing the chunk's backward buffer. This process typically reduces the memory requirement to $O(|c|n)$ for most window instances. \\
\textbf{Revision:} We add new experiments on memory consumption and discussion of the results of all approaches using all datasets in Section \ref{sec:memory_udage}. The memory experiments include all settings of our experiments, \textit{i.e.}, a sliding window with a window size of $3$M edges and $150$K edges, sliding windows with a slide size of $1$M edges and different window sizes, and sliding windows with a window size of $80$M edges and different slide sizes, excluding the workload size setting. Workload sizes were omitted as they do not impact memory usage, given that queries are processed through straightforward index lookups. In addition, we add discussion on the space complexity of our approach and compare it to the space complexity of FDC approaches at the end of Section \ref{sec:backward_parallel}. 
\smallskip
\smallskip
\smallskip

\textit{\textbf{D5.1}. In Section 7, only one of the experimental datasets overlaps with the most recent baseline, D-tree. It is recommended to include datasets such as youtube-growth and Semantic Scholar to align with the datasets and conduct a comprehensive performance comparison.}\\
\textbf{Answer:} %Thank you for the comment. 
We add Youtube-Growth (YG) and Semantic Scholar (SC) in the revised experimental evaluation, including throughput and latency evaluation (Figure \ref{fig:per_throughput} and Figure \ref{fig:per_latency}), scalability analysis with different window sizes (Figure \ref{fig:scale_window_size}), scalability analysis with slide intervals (Figure \ref{fig:scale_slide_size}), and scalability analysis with workload sizes (Figure \ref{fig:scale_workload_size}). Please notice that  Youtube-Growth is a small dataset with only $14.4$ million edges and our experiments regarding scalability analysis are focused on the case with window sizes up to $80$ million edges. Therefore, Youtube-Growth is infeasible for testing scalability. Semantic Scholar, having $8.27$ billion edges, allows us to conduct experiments on all these settings. 
Generally, our experimental results remain consistent over these two datasets, as shown in these figures. 
In addition, Youtube-Growth and Semantic Scholar are also included in the new experiments focused on reporting memory consumption (Figure \ref{fig:per-memory}).
\\
\textbf{Revision:} We conduct our experiments using Youtube-Growth (YG) and Semantic Scholar (SC), and the results have been added in Section \ref{sec:performance}, \textit{i.e.}, all figures have been updated by incorporating the results over the new datasets. Please see the answer to this comment for details. 
\smallskip
\smallskip
\smallskip

\textit{\textbf{D5.2}. Additionally, consider analyzing the results based on the characteristics of the datasets. 
Explore potential reasons for the impact on actual performance, including an examination of the dataset diameter's influence on results. According to the D-tree paper, performance is affected by diameter; therefore, investigate whether D-tree's performance is likely to surpass the BIC index on datasets with a smaller diameter.}\\
\textbf{Answer:} 
Please note that the characteristic of graphs, which is analyzed in the D-tree paper, is \textbf{average distance}, instead of diameter. 
Although average distance is upper-bounded by diameter, they are  different. 
We report average distance and diameter of graphs in Section \ref{sec:exp_setup} and discuss the results based on it in Section \ref{sec:performance} . 
Please find below for the detailed explanation. 
% 
According to the experimental evaluation and discussion in the D-tree paper, average distance $avg_{sp}$ affects D-tree's performance and D-tree performs well in graphs with small $avg_{sp}$  (see Section 7.4 in the D-tree paper). Average distance is computed as the average sum of lengths of the shortest paths over all pairs of vertices, which is upper-bounded by diameter. 
This is because the design of D-tree takes into account the average distance from each vertex to its root in a spanning tree (Theorem 5.12 in the D-tree paper).
% 
However, the average distances of graphs do not have an impact on BIC because the BIC approach is based on Union-Find Trees, instead of spanning trees. Therefore, BIC does not perform BFS on graphs in the windows to process queries and index updates. 
In the revised experimental evaluation, we report the average distances of graphs that are available on the KONECT Project website. Notice that computing average distance is extremely expensive because it requires computing the shortest path distance for any pair of vertices in the graph, and this is the reason why the D-tree paper conducts the average distance analysis only on a synthetic graph with $480$ vertices (see Section 7.4 in the D-tree paper). 
The average distances of the graphs included in the experimental evaluation are very small, around $5$, which means these graphs are the best scenarios of D-tree. The average distances of the other graphs are expected to be small because of their power-low characteristics. 
Overall, BIC significantly outperforms D-tree in these real-world graphs that have very small average distances. \\
\textbf{Revision}: Average distance and diameter are very expensive to compute (see the answer to this comment for details). Therefore, we update Table \ref{table:datasets} to include average distance and diameter for some graphs for which these metrics are available. Then, at the end of Section \ref{sec:performance}, we add discussion related to them.
}
